INCLUDE: Evaluating Multilingual Language Understanding with Regional Knowledge

The performance differential of large language models (LLM) between languages hinders their effective deployment in many regions, inhibiting the potential economic and societal value of generative AI tools in many communities. However, the development of functional LLMs in many languages (\ie, multilingual LLMs) is bottlenecked by the lack of high-quality evaluation resources in languages other than English. Moreover, current practices in multilingual benchmark construction often translate English resources, ignoring the regional and cultural knowledge of the environments in which multilingual systems would be used. In this work, we construct an evaluation suite of 197,243 QA pairs from local exam sources to measure the capabilities of multilingual LLMs in a variety of regional contexts. Our novel resource, INCLUDE, is a comprehensive knowledge- and reasoning-centric benchmark across 44 written languages that evaluates multilingual LLMs for performance in the actual language environments where they would be deployed.

==> tables/main_results.tex <==
\section{Results \& Analysis}

\begin{table}[t]
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccc}
    \toprule
        & &\multicolumn{3}{c}{\textbf{\ourdatatiny}} & \multicolumn{3}{c}{\textbf{\ourdatalite}}\\
        \cmidrule(lr){3-5}\cmidrule(lr){6-8} 
        \textbf{Model} & 
\makecell{\textbf{\#} \\ \textbf{Langs}} & 
\makecell{\textbf{Total} \\ \textbf{Acc.}} & 
\makecell{\textbf{Answer} \\ \textbf{Acc.}} & 
\makecell{\textbf{Format} \\ \textbf{Errors (\%)}} & 
\makecell{\textbf{Total} \\ \textbf{Acc.}} & 
\makecell{\textbf{Answer} \\ \textbf{Acc.}} & 
\makecell{\textbf{Format} \\ \textbf{Errors (\%)}} \\
\midrule
        \textbf{GPT-4o} &   &   &   &   &  &  & \\
        - 5-shot &  & 77.5	& \textbf{82.7} & 6.3 & 77.3 &  \textbf{83.2} & 7.1 \\
        - Zero-shot CoT & & \textbf{78.8}  & 79.0 & 0.2 &  \textbf{79.0} &  79.2 & 0.2 \\

        \textbf{C4AI-Aya-23-35b} & 21 &   &   &   &  &  &  \\
        - 5-shot &  & 51.8 & 54.5 & 4.9 & 51.9 & 54.4 & 4.7 \\
        - Zero-shot CoT & & 43.3 & 49.3 & 12.3 & 45.7 & 50.0 & 11.1 \\

        \addlinespace[1ex]\cdashline{1-8}\addlinespace[1ex]
        \textbf{Aya-23-8B} & 21 & 32.5 & 42.1  & 22.8 & 34.0 & 42.6	& 20.1 \\

        \textbf{Mistral-7B (v0.3)} & - & 44.1 & 44.1 & 0.0 &  43.3  & 43.3 & 0.0  \\
        \textbf{Mistral-7B-Instruct (v0.3)} & - & 43.8 & 44.0 & 0.3 & 43.6 &  43.8 & 0.4\\
        
       \textbf{Gemma-7B} & - & \textbf{55.1} & \textbf{55.1} & 0.0 & \textbf{54.5}  & 54.5 & 0.0   \\
        \textbf{Gemma-7B-Instruct} & - & 39.1& 39.1 & 0.0 & 38.7  & 38.7 & 0.0  \\
        
        \textbf{Qwen2.5-7B} & 22 & 53.8 & 54.7 & 1.6 & 54.1 &  \textbf{55.1} & 1.9\\
        \textbf{Qwen2.5-7B-Instruct} & 22 & 53.2 & 53.4 & 0.4 &  53.8 & 54.0 & 0.5\\
        \textbf{Qwen2.5-14B}         & 22 & \textbf{60.9} & \textbf{61.8} & 1.4 & \textbf{61.4} & \textbf{62.4} & 1.5 \\
        
        \textbf{Llama-3-8B} & - & 50.0 & 50.0 & 0.0 & 50.3 &  50.3 & 0.0\\
        \textbf{Llama-3-8B-Instruct} & - & 49.9 & 49.9 & 0.0 & 49.8 &  49.8 & 0.0\\
        
        \textbf{XGLM-7.5B} & 23 & 25.3 & 26.4 & 4.0 & 25.0  & 26.1 & 4.1\\
        
        \textbf{BLOOM-7.1B} & 20 & 25.8 & 26.6 & 2.8 & 25.4 & 26.1 & 2.8  \\
        \textbf{BLOOMZ-7.1B} & 20 & 27.8 & 28.8 & 3.4 & 27.8 & 28.8 & 3.6  \\
        \bottomrule
    \end{tabular}}
    \caption{Results on \ourdatatiny{} and \ourdatalite{}. \textbf{Total Accuracy} represents the raw accuracy of the model for answering \ourdata{} questions in each respective subset. \textbf{Answer Accuracy} represents the accuracy of the model when only considering samples where an answer is extracted from the model's output in the correct response format. \textbf{Formatting Errors (\%)} describes the \% of model responses that are not formatted correctly and so do not output any answer option. We mark these incorrect by default in \textbf{Total Accuracy} and do not include them when computing \textbf{Answer Accuracy}. \textbf{\# Langs} reports the number of languages from \ourdata{} publicly reported to be \textit{intentionally} included in the pretraining data of each model. \nf{only keep the Qwen14B bold}}
    \label{tab:results}
\end{table}
